GGPT: Geometry Grounded Point Transformer

Recent feed-forward networks have achieved remarkable progress in sparse-view 3D reconstruction by predicting dense point maps directly from RGB images. However, they often suffer from geometric inconsistencies and limited fine-grained accuracy due to the absence of explicit multi-view constraints. We introduce the Geometry-Grounded Point Transformer (GGPT), a framework that augments feed-forward reconstruction with reliable sparse geometric guidance. We first propose an improved Structure-from-Motion pipeline based on dense feature matching and lightweight geometric optimisation to efficiently estimate accurate camera poses and partial 3D point clouds from sparse input views. Building on this foundation, we propose a geometry-guided 3D point transformer that refines dense point maps under explicit partial-geometry supervision using an optimised guidance encoding. Extensive experiments demonstrate that our method provides a principled mechanism for integrating geometric priors with dense feed-forward predictions, producing reconstructions that are both geometrically consistent and spatially complete, recovering fine structures and filling gaps in textureless areas. Trained solely on ScanNet++ with VGGT predictions, GGPT generalises across architectures and datasets, substantially outperforming state-of-the-art feed-forward 3D reconstruction models in both in-domain and out-of-domain settings.

==> fig/exp_cmp_completion.tex <==
\begin{figure}[h]
    \centering
    \fbox{
        \begin{minipage}[c][5cm][c]{8cm}
            \centering
            \textbf{Figure Placeholder}\\[0.5em]
            (Visual Results comparing ours and other completion methods \TODO{Nov 9})
        \end{minipage}
    }
    \caption{Caption for the figure.}
    \label{fig:cmp_completion}
\end{figure}

==> tab/ablation_SfM-matcher_RoMa-v2.tex <==
\begin{table*}[h!]
    \centering
    \small
\caption{\textbf{Ablation of SfM Components on all datasets.} For each variant, we report: (1) \textbf{Time} denotes the running time (s $\downarrow$) of each stage. (2) \textbf{Cam.} denotes the AUC@1/5$\degree$ (\% $\uparrow$) for camera-pose estimation. (3) \textbf{Pts.} (\% $\uparrow$) denotes the Accuracy/Completeness@1 cm (\% $\uparrow$) of reconstructed points.}

    \label{tab:ablate_sfm-matcher_romav2} 
    \vspace{-0.5em}
\setlength{\tabcolsep}{0.5pt} 
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l ccc c ccc c ccc @{}}
    \toprule
    & \multicolumn{3}{c}{4 Views} && \multicolumn{3}{c}{8 Views} && \multicolumn{3}{c}{16 Views} \\
    \cmidrule(lr){2-4} \cmidrule(lr){6-8} \cmidrule(lr){10-12}
    % & Time (s) $\downarrow$ & Cam. (\%) $\uparrow$ & Pts. (\%) $\uparrow$
    % && Time (s) $\downarrow$ & Cam. (\%) $\uparrow$ & Pts. (\%) $\uparrow$
    % && Time (s) $\downarrow$ & Cam. (\%) $\uparrow$ & Pts. (\%) $\uparrow$ \\
    & Time (s)  & Cam. (\%)  & Pts. (\%)
    && Time (s) & Cam. (\%) & Pts. (\%)
    && Time (s) & Cam. (\%) & Pts. (\%) \\
    \midrule
        (a) \textbf{ETH3D}   \\
        MASt3R~\cite{mast3r_eccv24} (Sparse) & 8.4 & 75/86 & 19/ \ 2 && 21 & 75/85 & 21/ \ 4 && 57 & 76/86 & 26/ \ 8 \\
        RoMa~\cite{edstedt2024roma} (Dense) & 2.3 & 90/93 & 47/20 && 8.8 & 87/91 & 46/25 && 36 & \textbf{89}/93 & 46/29 \\
        UFM~\cite{zhang2025ufm} (Dense) & \textbf{1.0} & 64/84 & 26/19 && \textbf{1.7} & 81/90 & 30/25 && \textbf{8.5} & 77/87 & 33/30 \\
        RoMa~\cite{edstedt2024roma} + UFM~\cite{zhang2025ufm} (Ours, Dense) & 3.3 & 86/93 & 35/22 && 11 & 87/92 & 37/30 && 44 & 85/91 & 40/35  \\
        \EXP{RoMav2} (Dense) & 2.2  & \textbf{95/98}  & \textbf{52/36} 
    && 8.1 & 92/\textbf{94} & \textbf{51/42} 
    && 36 & 88/94 & \textbf{54/47} \\ % outputs/benchmark_match/romav2/ma_eth3d/vggt/ba_2048-romav2/geo_results_for_pt3d
        \hdashline
        (b) \textbf{ScanNet++}   \\
        RoMa~\cite{edstedt2024roma} (Dense) &  Time  & 63/78 & 80/21  &&  Time  & 67/84 & 80/32  &&  Time  & 79/91 & 81/43 \\
        UFM~\cite{zhang2025ufm} (Dense) & Time  & 65/85 & 71/46  &&  Time  & 70/86 & 75/62  &&  Time  & 75/90 & 80/73 \\
        RoMa~\cite{edstedt2024roma} + UFM~\cite{zhang2025ufm} (Ours, Dense) & Time  & 69/86 & 74/48  &&  Time  & 72/88 & 76/63  &&  Time  & 78/91 & 80/75 \\
        \EXP{RoMav2} (Dense) & Time  & \textbf{83/92} & \textbf{81/53}  &&  Time  & \textbf{80/92} & \textbf{84/68}  &&  Time  & \textbf{83/93} & \textbf{87/77} \\ 
        \hdashline
        (c) \textbf{TandT}   \\
        RoMa~\cite{edstedt2024roma} (Dense) & Time  & 81/88 & 76/40  &&  Time  & 82/90 & 80/52  &&  Time  & 85/91 & 81/59 \\
        UFM~\cite{zhang2025ufm} (Dense) & Time  & 74/88 & 64/48  & & Time  & 80/90 & 69/62  &&  Time  & 80/89 & 73/69 \\
        RoMa~\cite{edstedt2024roma} + UFM~\cite{zhang2025ufm} (Ours, Dense) & Time  & 83/91 & 71/53  &&  Time  & 84/91 & 74/66  &&  Time  & 83/91 & 77/74 \\
        \EXP{RoMav2} (Dense) & Time  & \textbf{90/95} & \textbf{79/59}  &&  Time  & \textbf{88/93} & \textbf{82/71}  &&  Time  & \textbf{86/92} & \textbf{84/77}  \\ 
        \hdashline   
        (d) \textbf{4DDS}   \\
        RoMa~\cite{edstedt2024roma} (Dense) & \\
        UFM~\cite{zhang2025ufm} (Dense) &  \\
        RoMa~\cite{edstedt2024roma} + UFM~\cite{zhang2025ufm} (Ours, Dense) & \\
        \EXP{RoMav2} (Dense) &  \\ 
        \hdashline  
        (e) \textbf{MV-dVRK}   \\
        RoMa~\cite{edstedt2024roma} (Dense) & \\
        UFM~\cite{zhang2025ufm} (Dense) &  \\
        RoMa~\cite{edstedt2024roma} + UFM~\cite{zhang2025ufm} (Ours, Dense) & \\
        \EXP{RoMav2} (Dense) &  \\  
        \bottomrule
    \end{tabular*}
\end{table*}

        % /iopsstor/scratch/cscs/cyutong/code/PTv3_VGGT/outputs/local/scannet_from-roma_20k_r1.0_2nodes (reset radius to re-run)

==> tab/benchmark_short_breakdown.tex <==
\begin{table*}[ht!]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4pt} 
    \caption{\textbf{Multi-view 3D Reconstruction on Standard Test Sets.}
    We report AUC@5/10 cm (\% $\uparrow$). Our method (our SfM and GGPT) can improve dense predictions of various models. Despite GGPT is trained solely on ScanNet++ and VGGT's dense prediction, as we highlight the top-left cells as \dsid{within-domain}, it generalises well to \dscd{cross-domain datasets} and other methods' predictions (rows 3–10).}
    \centering
    \label{tab:ma_benchmark_breakdown}
    % \vspace{-0.5em}
\begin{tabular}{l cccccc c cccccc c cccccc}
\toprule
& \multicolumn{6}{c}{\dsid{ScanNet++}~\cite{yeshwanth2023scannet++}} 
&& \multicolumn{6}{c}{\dscd{ETH3D}~\cite{schoeps2017eth3d}}
&& \multicolumn{6}{c}{\dscd{T\&T}~\cite{Knapitsch2017tandt}} \\
& \multicolumn{2}{c}{4 imgs} & \multicolumn{2}{c}{8 imgs} & \multicolumn{2}{c}{16 imgs} && \multicolumn{2}{c}{4 imgs} & \multicolumn{2}{c}{8 imgs} & \multicolumn{2}{c}{16 imgs} && \multicolumn{2}{c}{4 imgs} & \multicolumn{2}{c}{8 imgs} & \multicolumn{2}{c}{16 imgs} \\
& w & wo & w & wo & w & wo &&
w & wo & w & wo & w & wo &&
w & wo & w & wo & w & wo \\
\midrule
SfM & 49/64 & 0/0&52/67 & 0/0&56/72 & 0/0&&55/70 & 0/0&56/70 & 0/0&57/71 & 0/0&&38/52 & 0/0&46/60 & 0/0&45/59 & 0/0 \\
VGGT~\cite{wang2025vggt} 
& 24/39 & 20/33&21/35 & 14/26&18/31 & 9/20&&29/44 & 22/33&24/39 & 16/26&21/33 & 12/21&&27/42 & 12/22&25/41 & 12/21&24/39 & 8/17 \\
~\cite{wang2025vggt} + Ours 
& 51/65 & 25/41&54/68 & 27/44&57/73 & 29/47&&52/68 & 21/32&55/69 & 20/32&55/70 & 18/30&&39/52 & 12/22&46/61 & 14/24&45/58 & 11/21 \\

\bottomrule
\end{tabular}

\end{table*}


\begin{table}[t!]
    \centering
    \small
\caption{\textbf{Multi-view 3D reconstruction on \dsod{out-of-domain} datasets.}  
AUC@1/5 cm (\% $\uparrow$) for human body reconstruction (4D-DRESS~\cite{wang20244ddress}) and AUC@1/5 mm (\% $\uparrow$) for surgical scene reconstruction (MV-dVRK~\cite{dvrk-smv}).}
  
    % colors indicate the \colorbox[RGB]{\colorfirst}{1st}, \colorbox[RGB]{\colorsecond}{2nd}, and \colorbox[RGB]{\colorthird}{3rd} best-performing model 
    \label{tab:ood_benchmark_breakdown}
    \vspace{-1em}

    \begin{tabular}{l cc c cc}
    \toprule
    % & \multicolumn{2}{c}{\textbf{\dsod{Out-of-domain}}}\\
    % \cmidrule(lr){2-3} 
    &\multicolumn{2}{c}{\footnotesize\textbf{\dsod{4D-DRESS}~\cite{wang20244ddress}}}  &&  \multicolumn{2}{c}{\footnotesize\textbf{\dsod{MV-dVRK}~\cite{dvrk-smv}}}\\
    & w & wo && w & wo \\
\midrule
SfM & 85/87 & 0/0&&62/73 & 0/0 \\
VGGT~\cite{wang2025vggt} & 12/42 & 7/32&&12/35 & 3/19 \\
~\cite{wang2025vggt} + Ours & 84/87 & 20/48&&63/73 & 15/35 \\


    \bottomrule
    \end{tabular}


\end{table}


==> tab/cmp_sfm.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4pt}
\footnotesize
    \centering
        \begin{tabular}{l c c cc }
        \toprule
     4 views   & Speed  (s)  & Extrinsics & Accuracy &  Completeness  \\
      & Time $\downarrow$ & AUC@1/5$\degree$ $\uparrow$ &  AUC@1/2/5 cm $\uparrow$ & AUC@1/2/5 cm $\uparrow$  \\
        \midrule
        %/iopsstor/scratch/cscs/cyutong/code/GeoGuided_3DLearning/run_eval_sfm.py
    COLMAP~\cite{colmap} &  \\
    VGG-SfM~\cite{wang2024vggsfm} & 9 &64/75& 5/9/21& 0/0/0 \\
    VGGT+BA~\cite{wang2025vggt} & 11 &57/78& 29/52/80& 0/1/4 \\
    MASt3R-SfM~\cite{duisterhof2025mastrsfm}& 21 &88/92& 22/43/69& 21/45/73\\
    Our SfM &  5 &90/94& 36/64/86& 24/46/63\\
    \midrule
     8 views   \\
        \midrule
    COLMAP~\cite{colmap} &  \\
    VGG-SfM~\cite{wang2024vggsfm} & 44 &60/68& 4/9/19& 0/0/1 \\
    VGGT+BA~\cite{wang2025vggt} & 42 &48/66& 26/46/70& 0/2/8 \\
    MASt3R-SfM~\cite{duisterhof2025mastrsfm}& 52 &79/83& 24/44/66& 23/46/72  \\
    Our SfM & 15 &89/93& 38/65/86& 32/55/73 \\
    \midrule
     16 views  \\
        \midrule
    COLMAP~\cite{colmap} &  \\
    VGG-SfM~\cite{wang2024vggsfm}& 89 &38/47& 2/5/11& 0/0/0  \\
    VGGT+BA~\cite{wang2025vggt} & 176 &41/57& 28/47/70& 1/3/12 \\
    MASt3R-SfM~\cite{duisterhof2025mastrsfm}& 115 &76/82& 27/49/73& 26/52/79\\
    Our SfM & 60 &85/91& 40/68/89& 35/62/80\\

        \bottomrule
        \end{tabular}
    \caption{\textbf{Comparison between our and other SfM methods on ETH3D~\cite{schoeps2017eth3d}.} Our SfM method provides the best trade-off between accuracy, completeness, and efficiency, surpassing prior works such as MASt3R-SfM~\cite{duisterhof2025mastrsfm} in both reconstruction accuracy and computational speed.}
    \label{tab:cmp_sfm}
\end{table}

% \begin{table}[h]
% \setlength{\tabcolsep}{4pt}
% \footnotesize
%     \centering
%         \begin{tabular}{l c c ccc}
%         \toprule
%      4 views   & Speed  (s)  & Camera & \multicolumn{3}{c}{Points Error (cm)}   \\
%       & Time $\downarrow$ & AUC@5/10$\degree$ $\uparrow$ &  Acc. $\downarrow$& Com.  $\downarrow$  & Avg. $\downarrow$ \\
%         \midrule
%         %/iopsstor/scratch/cscs/cyutong/code/GeoGuided_3DLearning/run_eval_sfm.py
%     COLMAP~\cite{colmap} &  \\
%     VGG-SfM~\cite{wang2024vggsfm} & 9 &76/78& 28&261&145  \\
%     VGGT+BA~\cite{wang2025vggt} & 11 &66/75& 2.5&68&35  \\
%     MASt3R-SfM~\cite{duisterhof2025mastrsfm}& 21 &92/94&3.1&2.8&2.9  \\
%     Our SfM &  5 &94/96&1.7&7.3&4.5  \\
%     \midrule
%      8 views   \\
%         \midrule
%     COLMAP~\cite{colmap} &  \\
%     VGG-SfM~\cite{wang2024vggsfm} & 44 &68/70& 39& 260& 150\\
%     VGGT+BA~\cite{wang2025vggt} & 42 &66/74& 3.0&60&32   \\
%     MASt3R-SfM~\cite{duisterhof2025mastrsfm}& 52 &83/85& 6.2&4.0&5.0  \\
%     Our SfM & 15 &93/95& 1.7&4.3 &3.0 \\
%     \midrule
%      16 views  \\
%         \midrule
%     COLMAP~\cite{colmap} &  \\
%     VGG-SfM~\cite{wang2024vggsfm}& 89 &57/50& 330&229&255\\
%     VGGT+BA~\cite{wang2025vggt} & 176 &57/65& 4.4&30&17\\
%     MASt3R-SfM~\cite{duisterhof2025mastrsfm}& 115 &82/83& 2.5&2.2&2.3 \\
%     Our SfM & 60 &91/94& 1.4&1.6&1.5 \\

%         \bottomrule
%         \end{tabular}
%     \caption{\textbf{Comparison between our and other SfM methods on ETH3D~\cite{schoeps2017eth3d}.} Our SfM method provides the best trade-off between accuracy, completeness, and efficiency, surpassing prior works such as MASt3R-SfM~\cite{duisterhof2025mastrsfm} in both reconstruction accuracy and computational speed.}
%     \label{tab:cmp_sfm}
% \end{table}

